CFD analysis of electroviscous effects in electrolyte liquid flow through heterogeneously charged uniform microfluidic device

This study has numerically investigated the charge-heterogeneity effects in the electroviscous flow of symmetric ($1$:$1$) electrolyte liquid through a uniform slit microfluidic device. The Poisson's, Nernst-Planck (N-P), Navier-Stokes (N-S), and continuity equations are solved using the finite element method (FEM) to obtain the flow fields, such as total electrical potential ($U$), excess charge ($n^\ast$), induced electric field strength ($E_\text{x}$), and pressure ($P$) fields for following conditions: inverse Debye length ($2\le K\le 20$), surface charge density ($4\le \mathit{S_\text{1}}\le 16$), and surface charge-heterogeneity ratio ($0\le \mathit{S_\text{rh}}\le 2$). Results have shown that the total potential ($|\Delta U|$) and pressure ($|\Delta P|$) drop maximally increase by 99.09% (at $K=20$, $\mathit{S_\text{1}}=4$) and 12.77% (at $K=2$, $\mathit{S_\text{1}}=8$), respectively with overall charge-heterogeneity ($0\le \mathit{S_\text{rh}}\le 2$). Electroviscous correction factor (i.e., the ratio of effective to physical viscosity) maximally enhances by 12.77% (at $K=2$, $\mathit{S_\text{1}}=8$), 40.98% (at $\mathit{S_\text{1}}=16$, $\mathit{S_\text{rh}}=1.50$), and 41.35% (at $K=2$, $\mathit{S_\text{rh}}=1.50$), with the variation of $\mathit{S_\text{rh}}$ (from 0 to 2), $K$ (from 20 to 2), and $\mathit{S_\text{1}}$ (from 0 to 16), respectively. Further, a simple pseudo-analytical model is developed to estimate the pressure drop in the electroviscous (EV) flow, accounting for the influence of charge-heterogeneity based on the Poiseuille flow in the uniform channel. This model predicts the pressure drop $\pm$2-4% within the numerical results. The robustness and simplicity of this model enable the present numerical results for engineering and design aspects of microfluidic applications.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~



